Load Balancing for Skewed Streams on Heterogeneous Cluster

Streaming applications frequently encounter skewed workloads and execute on heterogeneous clusters. Optimal resource utilization in such adverse conditions becomes a challenge, as it requires inferring the resource capacities and input distribution at run time. In this paper, we tackle the aforementioned challenges by modeling them as a load balancing problem. We propose a novel partitioning strategy called Consistent Grouping (CG), which enables each processing element instance (PEI) to process the workload according to its capacity. The main idea behind CG is the notion of small, equal-sized virtual workers at the sources, which are assigned to workers based on their capacities. We provide a theoretical analysis of the proposed algorithm and show via extensive empirical evaluation that our proposed scheme outperforms the state-of-the-art approaches, like key grouping. In particular, CG achieves 3.44x better performance in terms of latency compared to key grouping.

==> sections/applications.tex <==
% !TEX root =  ../main.tex
\section{Applications}
\label{sec:applications}
%\note{Anis- this section provides some example application. We can get rid of this section if needed.}
Consistent grouping follows the same programming primitive as \pkgs for stream partitioning. % and not every algorithm can be expressed with it.
%In general, all algorithms that use shuffle grouping can use \cg to reduce their memory footprint.
%In addition, many algorithms expressed via key grouping can be rewritten to use \cg in order to get better load balancing.
In this section we provide a few such examples of common data mining algorithms, and show the advantages of \cg. % in terms of load balancing, memory consumption, or approximation error.
%Henceforth, we assume that each message contains a data point for the application, e.g., a feature vector in a high-dimensional space.

%\subsection{Na\"{i}ve Bayes Classifier}
%A na\"{i}ve Bayes classifier is a probabilistic model that assumes independence of features.
%It estimates the probability of a class $C$ given a feature vector $X$ by using Bayes' theorem.
%In practice, the classifier works by counting the frequency of co-occurrence of each feature and class values.
%
%The simplest way to parallelize this algorithm is to spread the counters across several workers via vertical parallelism, i.e., each feature is tracked independently in parallel.
%Following this design, the algorithm can be implemented by the same pattern used for the \kg example in Section~\ref{sec:existing-partitioning}. %Figure~\ref{fig:wordcounts}(a).
%Sparse datasets often have a skewed distribution of features, e.g., for text classification.
%Therefore, this implementation suffers from the same load imbalance, which \pkgs solves.
%
%Horizontal parallelism can also be used to parallelize the algorithm, i.e., by shuffling messages to separate workers.
%This implementation uses the same pattern as the \dagr in the \sg example in Section~\ref{sec:existing-partitioning}. %Figure~\ref{fig:wordcounts}(b).
%The count for a single feature-class pair is distributed across several workers, and needs to be combined at prediction (query) time. % in order to get the final classification.
%This combination requires broadcasting the query to all the workers, as a feature can be tracked by any worker.
%This implementation, while balancing the work better than key grouping, requires an expensive query stage that may be affected by stragglers.

\subsection{Streaming Parallel Decision Tree}

%\note[gdfm]{These sketches should NOT lose accuracy on merging}

A decision tree is a classification algorithm that uses a tree-like model where nodes are tests on features, branches are possible outcomes, and leafs are class assignments.

\citet{ben-haim2010spdt} propose an algorithm to build a streaming parallel decision tree that uses approximated histograms to find the test value for continuous features.
Messages are shuffled among $W$ workers.
Each worker generates histograms independently for its sub-stream, one histogram for each feature-class-leaf triplet.
These histograms are then periodically sent to a single aggregator that merges them to get an approximated histogram for the whole stream.
The aggregator uses this final histogram to grow the model by taking split decisions for the current leaves in the tree.
Overall, the algorithm keeps $W \times D \times C \times L$ histograms, where $D$ is the number of features, $C$ is the number of classes, and $L$ is the current number of leaves.

%One of the advantages of shuffle grouping is that each worker receives the same number of messages.
The memory footprint of the algorithm depends on $W$, so it is impossible to fit larger models by increasing the parallelism.
%The only way to reduce memory pressure is to reduce the accuracy of the histograms by reducing the number of bins.
Moreover, the aggregator needs to merge $W \times D \times C$ histograms each time a split decision is tried, and merging the histograms is one of the most expensive operations.

\subsection{Heavy Hitters and Space Saving}

The heavy hitters problem consists in finding the top-k most frequent items occurring in a stream.
The \textsc{SpaceSaving}~\citep{metwally2005spacesaving} algorithm solves this problem approximately in constant time and space.
Recently, \citet{berinde2010heavyhitters} have shown that \textsc{SpaceSaving} is space-optimal, and how to extend its guarantees to merged summaries.
This result allows for parallelized execution by merging partial summaries built independently on separate sub-streams.

In this case, the error bound on the frequency of a single item depends on a term representing the error due to the merging, plus another term which is the sum of the errors of each individual summary for a given item $i$:
$$
\mid \hat{f}_i - f_i \mid \leq \Delta_{f} + \sum_{j=i}^{W}\Delta_{j}
$$
where $f_i$ is the true frequency of item $i$ and $\hat{f}_i$ is the estimated one, each $\Delta_j$ is the error from summarizing each sub-stream, while $\Delta_{f}$ is the error from summarizing the whole stream, i.e., from merging the summaries.

Observe that the error bound depends on the parallelism level $W$.
Conversely, by using \kg, the error for an item depends only on a single summary, thus it is equivalent to the sequential case, at the expense of poor load balancing.

%\subsection{Hash-based Group-by Join}
%\emph{Hash-based Group-by} (\hg) is one of the important operations in relational database management systems.
%\hg operations are divided into two parts: \emph{hash join} and \emph{group by}.
%Consider that we are given two relations $\calR$ and $\calS$ that we desire to perform \hg on keys $a$ and $b$, i.e., $\text{group}(\calR.a = \calS.b)$.
%Further, we are given \numworkers processing elements (\pe) that are responsible for performing the join operation.
%Ideally, both $\calR$ and $\calS$ are distributed across the \pes in a way that each processing element receives nearly $\frac{\mid \calR\mid}{n}$ and $\frac{\mid \calS\mid}{n}$ rows.
%The \hg executes in three phases: build, probe and aggregate.  
%During the build phase, each \pe reads the rows from the smaller of the two relations and creates an in-memory hash table.  
%During the probe phase, each \pe locally reads all rows from the other relation, hashes these key on the same equijoin keys, and probes for matching rows in the hash table.
%Finally, during the aggregate phase, each \pe aggregates all the rows that corresponds to the same key.
%In case of parallel \hg, both the relations are distributed across the processing elements and the \hg is performed locally at each \pe.




==> sections/model.tex <==
% !TEX root =  ../loadBalancing.tex
%% MODEL
\section{Formal Model}
We want to model the decision of rebalancing an unbalanced system as a rent/buy problem (\url{http://en.wikipedia.org/wiki/Ski_rental_problem}).
The cost of renting is the cost of perdured imbalance.
The cost of buying is the cost of performing the rebalancing.

One way to see the analogy is to thing about the following problem.
\begin{quote}
Total completion time scheduling: We wish to schedule jobs with fixed processing times on m identical machines. The processing time of job j is pj. Each job becomes known to the scheduler on its release time rj. The goal is to minimize the sum of completion times over all jobs. A simplified problem is one single machine with the following input: at time 0, a job with processing time 1 arrives; k jobs with processing time 0 arrive at some unknown time. We need to choose a start time for the first job. Waiting incurs a cost of 1 per time unit, yet starting the first job before the later k jobs may incur an extra cost of k in the worst case. This simplified problem may be viewed as a continuous version of the ski rental problem.

Steven S. Seiden. A guessing game and randomized online algorithms. STOC '00.
\end{quote}

A 2-approximation algorithm for this problem is the break-even algorithm.
The algorithm choses to rent as long as the cumulative cost of renting is less than the cost of buying.
We can even do better with a randomized algorithm.


\mpara{Objective Function.}
We want to minimize the Maximum(latency).
For evaluation, we can measure (Max(l) - Avg(l))/Avg(l).

\mpara{Queuing Model.}
Assume the following model for the computation (similar to Flux).
There are S sources, W workers, P partitions of the stream (can be (hot) keys or groups of keys).
Each source has an outgoing queue per partition, and each worker has an incoming queue per partition.

\mpara{Rebalancing.}
The rebalancing algorithm can move one partition $p \in \mathcal{P}$ from one worker to another.
Alternatively, we can exchange two partitions between two workers.
When the rebalancing algorithm moves one partition, the worker drains its incoming queue.
Alternatively, it should migrate both the state of the operator and the incoming queue (depends on the service time).
At the same time, the outgoing queues for the migrating partition at the sources are stopped, i.e., they accumulate messages.
When the migration is over, the outgoing queues are restarted with the new worker as a destination.

\mpara{Costs.}
\begin{squishlist}
\item Latency = Time-enqueued - Time-served (for a single message)
\item Cost of renting = cost of imbalance = Max(latency) - Avg(latency) (across workers)
\item Cost of buying = cost of rebalancing = (Time-to-drain + Time-to-migrate) / ((Cost-of-renting - Cost-of-renting-after-migration)/Cost-of-renting)).
\end{squishlist}


\mpara{Partitions.}
How many partitions do we need?

\mpara{Routing.}
How do we keep the routing table?
If full routing table, then every migration is possible.
If it leverages the power-of-two-choices, then we need only $log_2(W)$ bits to store the routing table.
However, we can only migrate one partition to another possible place.


\mpara{Simulations for Baseline (Flux).}
Simulate Flux, and see if it reaches a steady state.
If it does, then there is no point in our paper :)


==> sections/pitch.tex <==
% !TEX root =  ../loadBalancing.tex
%% PITCH
\section{Motivation}


==> sections/problem-def.tex <==
%% PROBLEM DEFINITION
\section{Problem definition}


==> tikz-defines.tex <==
%%%%%%%%%%%%%%%%
%% tikz stuff %%
%%%%%%%%%%%%%%%%

\usepackage{tikz,pgfplots,pgfplotstable}
\usetikzlibrary{positioning,fit,shapes}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows}

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\makeatletter
\tikzset{multicircle/.style  args={#1, #2}{%
 alias=tmp@name, % 
  postaction={%
    insert path={
     \pgfextra{% 
     \pgfpointdiff{\pgfpointanchor{\pgf@node@name}{center}}%
                  {\pgfpointanchor{\pgf@node@name}{east}}%            
     \pgfmathsetmacro\insiderad{\pgf@x}%
     %\foreach \c [count=\ci from = 0, evaluate=\ci as \angle using 360 - (\ci) * #1] in {#2}%
        \fill[white] (\pgf@node@name.center)  circle (\insiderad-\pgflinewidth);%
        \draw[#2] (\pgf@node@name.center)  circle (\insiderad-\pgflinewidth);%
        \fill[#2] (\pgf@node@name.center)  -- ++(0:\insiderad-\pgflinewidth) arc (0:#1:\insiderad-\pgflinewidth)--cycle;%
        }}}}}
\makeatother

\definecolor{yafaxiscolor}{rgb}{0.3, 0.3, 0.3}
\definecolor{yafcolor1}{rgb}{0.4, 0.165, 0.553}
\definecolor{yafcolor2}{rgb}{0.949, 0.482, 0.216}
\definecolor{yafcolor3}{rgb}{0.47, 0.549, 0.306}
\definecolor{yafcolor4}{rgb}{0.925, 0.165, 0.224}
\definecolor{yafcolor5}{rgb}{0.141, 0.345, 0.643}
\definecolor{yafcolor6}{rgb}{0.965, 0.933, 0.267}
\definecolor{yafcolor7}{rgb}{0.627, 0.118, 0.165}
\definecolor{yafcolor8}{rgb}{0.878, 0.475, 0.686}
\definecolor{yafcolor9}{rgb}{0.965, 0.733, 0.767}

\newlength{\yafaxispad}
\setlength{\yafaxispad}{-4pt}
\newlength{\yaftlpad}
\setlength{\yaftlpad}{\yafaxispad}
\addtolength{\yaftlpad}{-0pt}
\newlength{\yaflabelpad}
\setlength{\yaflabelpad}{-2pt}
\newlength{\yafaxiswidth}
\setlength{\yafaxiswidth}{1.2pt}
\newlength{\yafticklen}
\setlength{\yafticklen}{2pt}

\makeatletter
\def\pgfplots@drawtickgridlines@INSTALLCLIP@onorientedsurf#1{}
\makeatother

\newcommand{\yafdrawxaxis}[2]{
  \pgfplotstransformcoordinatex{#1}\let\xmincoord=\pgfmathresult 
  \pgfplotstransformcoordinatex{#2}\let\xmaxcoord=\pgfmathresult 
  \pgfsetlinewidth{\yafaxiswidth} 
  \pgfsetcolor{yafaxiscolor}
  \pgfpathmoveto{\pgfpointadd{\pgfpointadd{\pgfplotspointrelaxisxy{0}{0}}{\pgfqpointxy{\xmincoord}{0}}}{\pgfqpoint{-0.5\yafaxiswidth}{\yafaxispad}}}
  \pgfpathlineto{\pgfpointadd{\pgfpointadd{\pgfplotspointrelaxisxy{0}{0}}{\pgfqpointxy{\xmaxcoord}{0}}}{\pgfqpoint{0.5\yafaxiswidth}{\yafaxispad}}}
  \pgfusepath{stroke}

}
\newcommand{\yafdrawyaxis}[2]{
  \pgfplotstransformcoordinatey{#1}\let\ymincoord=\pgfmathresult 
  \pgfplotstransformcoordinatey{#2}\let\ymaxcoord=\pgfmathresult 
  \pgfsetlinewidth{\yafaxiswidth} 
  \pgfsetcolor{yafaxiscolor}
  \pgfpathmoveto{\pgfpointadd{\pgfpointadd{\pgfplotspointrelaxisxy{0}{0}}{\pgfqpointxy{0}{\ymincoord}}}{\pgfqpoint{\yafaxispad}{-0.5\yafaxiswidth}}}
  \pgfpathlineto{\pgfpointadd{\pgfpointadd{\pgfplotspointrelaxisxy{0}{0}}{\pgfqpointxy{0}{\ymaxcoord}}}{\pgfqpoint{\yafaxispad}{0.5\yafaxiswidth}}}
  \pgfusepath{stroke}
}

\newcommand{\yafdrawaxis}[4]{\yafdrawxaxis{#1}{#2}\yafdrawyaxis{#3}{#4}}

\pgfplotscreateplotcyclelist{yaf}{% 
{yafcolor1,mark options={scale=0.75},mark=o}, 
{yafcolor2,mark options={scale=0.75},mark=square},
{yafcolor3,mark options={scale=0.75},mark=triangle},
{yafcolor4,mark options={scale=0.75},mark=o},
{yafcolor5,mark options={scale=0.75},mark=o},
{yafcolor6,mark options={scale=0.75},mark=o},
{yafcolor7,mark options={scale=0.75},mark=o},
{yafcolor8,mark options={scale=0.75},mark=o}} 

\pgfplotsset{axis y line=left, axis x line=bottom,
  tick align=outside,
  compat = 1.3,
  tickwidth=\yafticklen,
  clip = false,
  every axis title shift = 0pt,
    x axis line style= {-, line width = 0pt, opacity = 0},
    y axis line style= {-, line width = 0pt, opacity = 0},
    x tick style= {line width = \yafaxiswidth, color=yafaxiscolor, yshift = \yafaxispad},
    y tick style= {line width = \yafaxiswidth, color=yafaxiscolor, xshift = \yafaxispad},
    x tick label style = {font=\scriptsize, yshift = \yaftlpad},
    y tick label style = {font=\scriptsize, xshift = \yaftlpad},
    every axis y label/.style = {at = {(ticklabel cs:0.5)}, rotate=90, anchor=center, font=\scriptsize, yshift = -\yaflabelpad},
    every axis x label/.style = {at = {(ticklabel cs:0.5)}, anchor=center, font=\scriptsize, yshift = \yaflabelpad},
    x tick label style = {font=\scriptsize, yshift = 1pt},
    grid = major,
    major grid style  = {dash pattern = on 1pt off 3 pt},
  every axis plot post/.append style= {line width=\yafaxiswidth} ,
  legend cell align = left,
  legend style = {inner sep = 1pt, cells = {font=\scriptsize}},
  legend image code/.code={%
    \draw[mark repeat=2,mark phase=2,#1] 
    plot coordinates { (0cm,0cm) (0.15cm,0cm) (0.3cm,0cm) };% 
  } 
}

\newcommand{\cemph}[1]{{\color{yafcolor7}#1}}
\newcommand{\cact}[1]{{\color{aaltoblue}#1}}


